Perceived Trustworthiness of Natural Language Generators

Natural Language Generation tools, such as chatbots that can generate human-like conversational text, are becoming more common both for personal and professional use. However, there are concerns about their trustworthiness and ethical implications. The paper addresses the problem of understanding how different users (e.g., linguists, engineers) perceive and adopt these tools and their perception of machine-generated text quality. It also discusses the perceived advantages and limitations of Natural Language Generation tools, as well as users' beliefs on governance strategies. The main findings of this study include the impact of users' field and level of expertise on the perceived trust and adoption of Natural Language Generation tools, the users' assessment of the accuracy, fluency, and potential biases of machine-generated text in comparison to human-written text, and an analysis of the advantages and ethical risks associated with these tools as identified by the participants. Moreover, this paper discusses the potential implications of these findings for enhancing the AI development process. The paper sheds light on how different user characteristics shape their beliefs on the quality and overall trustworthiness of machine-generated text. Furthermore, it examines the benefits and risks of these tools from the perspectives of different users.

==> letter.tex <==
We would like to thank the reviewers for their sensible and highly useful comments, insights, and ideas for future work. Their comments are addressed as follows: 

\begin{itemize}
    \item ``As far as RRI goes this is not very deep as it focuses on the anticipation of ethical issues and not at all on other aspects of RRI, such as mitigation and action.'' This is a very good point and we are aware of how interesting the topic of mitigation and policy-making is. Nevertheless, we felt the need to keep the original scope. We also believe it would be interesting to replicate this work and extend it with the RRI rationales (now that the public opinion is somewhat settled).

    \item ``[...] improve the clarity of the background section (esp. sections about foundation models and legal frameworks)'' We reprhased some paragraphs to make them easier to follow. Moreover, in retrospective, we believed that it was more straightforward to title the paragraph about new NLG tools as ''language models'' and discuss the challenges of new tools based on ''foundation models''. The chatbot paragraph was moved up to exemplify how ''language models'' can be integrated into everyday devices.

    \item ``[...] building trust could lead to increased adoption is not particularly original'' we do not want to claim this, but highlight that trust (even if unjustified) can lead to increased use (including misuse)! The last sentence in 4.3 was changed to make this explicit.

    \item ``It was unclear why the views of non-expert users about compliance with GDPR was relevant?'' We believe that the views on GDPR (as a disruptive legislation that also affect non-expert participants) is very relevant for the discussion on ''ethical risks and mitigation regulations'' (6.3) and for participants to reflect on the meaning of trust (privacy also affects non-expert participants).

    \item ``[...] references to legal frameworks were vague and needed to cite the law rather than articles'' Yes, this was a concious decision as we did not want to go into details but to frame this work using the EU AI Act law draft. Comparing the scope of this law to other regulations would require further discussion (hopefully at TAS 23!).

    \item ``[...] It would have been interesting to relate the question around identifying sentences written by humans to issues of fraud/misinformation.'' Totally! However, this would require a new experiment. This is a very interesting line for future work, maybe working with news headlines. 

    \item ``[...] hard to follow which groups were being discussed and thus to relate the results to particular sectors'' We considered using names for different groups but the text felt very repetitive. We also considered calling groups (L)anguage, (T)echnology, and (O)thers but it was similarly difficult to follow. In the end, we decided to only remind the reader about the backgrounds of the groups when needed.

    \item ``[...] how the findings linked to specific measures to improve such tools for particular contexts'' 6.2 is meant to reflect on the participants' thoughts about this topics, however, further details are outside the scope of these work (yet a very interesting discussion topic that, based on the gathered responses, should also involve non-experts).

    \item ``[...] more detailed written explanations of the results rather than referring the reader to the tables'' We wrote what explanations we considered relevant for the 14 table references, but if you feel like any in particular is not as clear as it should be, please get in touch so we can reframe it. Thanks!

    \item ``[...] be more descriptive of the results within the text of the paper.'' and ''further thought as to how to express the results more impactfully'' Text slighly edited to take these comments into account. We hope now it's clearer.
\end{itemize}

\vspace{.5cm}


With best wishes, \\
The authors
